Characterizing Fairness Over the Set of Good Models Under Selective Labels

Algorithmic risk assessments are used to inform decisions in a wide variety of high-stakes settings. Often multiple predictive models deliver similar overall performance but differ markedly in their predictions for individual cases, an empirical phenomenon known as the "Rashomon Effect." These models may have different properties over various groups, and therefore have different predictive fairness properties. We develop a framework for characterizing predictive fairness properties over the set of models that deliver similar overall performance, or "the set of good models." Our framework addresses the empirically relevant challenge of selectively labelled data in the setting where the selection decision and outcome are unconfounded given the observed data features. Our framework can be used to 1) replace an existing model with one that has better fairness properties; or 2) audit for predictive bias. We illustrate these uses cases on a real-world credit-scoring task and a recidivism prediction task.

==> Fairness Frontier/Tables/Personal-Loans/applicantSummaryStatistics-table.tex <==
\begin{tabular}{ l | c c c c c c c }
    & \multicolumn{5}{c}{\textbf{Quantiles}} \\
    & 1\% & 5\% & 25\% & 50\% & 75\% & 95\% & 99\% \\
    \hline 
    & \multicolumn{5}{c}{\textbf{All Applications}} \\
    Total Net Income (\$AU)  & 15,599 & 20,672 & 32,039 & 41,370 & 53,831 & 86,984 & 135,191 \\
    Total Liabilities (\$AU)  & -341 & 0 & 0 & 2 & 6,700 & 225,195 & 546,982 \\
    Credit Bureau Score & 0	& 0 & 443 & 587 & 689 & 827 & 936 \\
    & \multicolumn{5}{c}{\textbf{Funded Applications}} \\
    Total Net Income (\$AU)  & 17,316 & 22,439 & 33,095 & 41,471 & 53,111 & 83,891 & 118,922 \\
    Total Liabilities (\$AU)  & -943 & 0 & 0 & 0 & 7,000 & 262,628 & 539,278 \\
    Credit Bureau Score & 367 & 464 & 586 & 661 & 741 & 863	& 958 \\
    & \multicolumn{5}{c}{\textbf{Disadvantaged Geographic Areas}} \\
    Total Net Income (\$AU) & 15,323 & 19,913 & 30,227 & 39,107 & 50,735 & 80,303 & 127,391 \\
    Total Liabilities (\$AU) & -203 & 0 & 0 & 0 & 5,650 & 162,000 & 420,000 \\
    Credit Bureau Score & 0 & 0 & 406 & 566 & 677 & 828 & 937 \\
    & \multicolumn{5}{c}{\textbf{Non-disadvantaged Geographic Areas}} \\
    Total Net Income (\$AU)  & 15,600 & 20,796 & 32,435 & 41,858 & 54,625 & 88,595 & 137,005 \\
    Total Liabilities (\$AU) & -389 & 0 & 0 & 3 & 7000 & 246,000 & 572,007 \\
    Credit Bureau Score & 0 & 0 & 454 & 593 & 692 & 826 & 935 
\end{tabular}


==> Fairness Frontier/Tables/Personal-Loans/loanPurpose-top10-table.tex <==
\begin{tabular}{l | c}
    \textbf{Loan Purpose} & \\
    \hline
    Used car & 31.6\% \\
    Refinance debt at other financial institution & 11.3\% \\
    Personal goods & 9.8\% \\
    Travel & 8.8\% \\
    New car & 6.2\% \\
    Other & 5.5\% \\
    Home Improvement & 5.1\% \\
    Other motor vehicle & 2.8\% \\
    Motor vehicle repairs & 2.8\% \\
    Land purchase & 2.5\%
\end{tabular}





==> Fairness Frontier/Tables/Personal-Loans/loanTermSummaryStatistics-table.tex <==
\begin{tabular}{l | c c c c c c c}
    & \multicolumn{5}{c}{\textbf{Quantiles}} \\
    & 1\% & 5\% & 25\% & 50\% & 75\% & 95\% & 99\% \\
    \hline
    Loan size (\$AU) & 4,000 & 4,000 & 5,000 & 10,000 & 17,800 & 35,000 & 50,000 \\
    Interest rate & 8.49 & 11.9 & 13.9 & 13.9 & 15.9 & 17.9	& 18.4 \\
    Loan size to net income ratio & 0.056 & 0.081 & 0.139 & 0.238 & 0.412 & 0.793 & 1.150 \\
    Savings balance to loan size ratio & 0.000 & 0.000 & 0.026	& 0.087 & 0.267 & 1.339 & 4.374 
\end{tabular}

==> Fairness Frontier/arXiv-Headers.tex <==
% Links
	\usepackage{hyperref}
%	\usepackage{cleveref}
	
\hypersetup{
    colorlinks=true,
    linkcolor=red,
    citecolor=blue,
    filecolor=magenta,      
    urlcolor=cyan,
}

% Typesetting
    \usepackage[T1]{fontenc}
	\usepackage[utf8]{inputenc}
	\usepackage[english]{babel}
	\usepackage{amsfonts}
	\usepackage{amssymb}
	\usepackage{amsthm}
	\usepackage{enumitem}
	\usepackage{bbm}
	\usepackage{mathtools}
	\usepackage{booktabs}	
	\usepackage{setspace}
	\usepackage{graphicx}
	\onehalfspacing
	\usepackage{fullpage}
	\def\labelitemi{--}
	\usepackage{soul}
	\usepackage{xspace}
	\usepackage{csquotes}
	\usepackage{changepage}
	\usepackage{verbatim}
    %\usepackage[tocflat]{tocstyle}
    \usepackage{placeins}
    
\usepackage{tikz}
\usepackage{subcaption}
\usepackage{textcomp}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{caption}
\usepackage{subcaption}
%\usepackage{hyperref}
%%
%% \BibTeX command to typeset BibTeX logo in the docs
\AtBeginDocument{%
  \providecommand\BibTeX{{%
    \normalfont B\kern-0.5em{\scshape i\kern-0.25em b}\kern-0.8em\TeX}}}

%% Rights management information. .
%\copyrightyear{2019}
%\acmYear{2019}
%\setcopyright{rightsretained}

\usepackage[suppress]{color-edits}
%\usepackage{color-edits}
\addauthor[Amanda]{am}{blue}
\addauthor[Alex]{ac}{purple}
\addauthor[Ashesh]{as}{green}

\newcommand{\p}{\mathbb{P}}
\newcommand{\e}{\mathbb{E}}
\newcommand{\eh}{\hat{\mathbb{E}}}
\newcommand{\reals}{\mathbb{R}}
\newcommand{\abs}[1]{\left| #1 \right|}

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\ty}{\tilde{y}}
\newcommand{\tu}{\tilde{u}}

\newcommand{\yh}{\hat{Y}}
\newcommand{\yT}{Y^{T=1}}
\newcommand{\yt}{Y^{1}}
\newcommand{\yD}{Y^{D=1}}
\newcommand{\yd}{Y^{1}}

\newcommand{\indep}{\perp \!\!\!\perp}
\newcommand{\loss}{\operatorname{loss}}
\newcommand{\cost}{\operatorname{cost}}
\newcommand{\unfair}{\operatorname{unfair}}
\newcommand{\FPI}{\operatorname{FPI}}
\newcommand{\disp}{\operatorname{disparity}}
\newcommand{\best}{\operatorname{Best}}

% Hat variables
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\costhat}{\widehat{\cost}}
\newcommand{\disphat}{\widehat{\disp}}
\newcommand{\lambdahat}{\hat \lambda}
\newcommand{\etahat}{\hat \eta}
\newcommand{\epsilonhat}{\hat \epsilon}
\newcommand{\hnuma}{\hat{\omega}_1}
\newcommand{\hnum}{\hat{\omega}}
\newcommand{\hnumo}{\hat{\omega}_0}
\newcommand{\hdena}{\hat{\bar{\omega}}_1}
\newcommand{\hdeno}{\hat{\bar{\omega}}_0}
\newcommand{\hden}{\hat{\bar{\omega}}}
\newcommand{\numa}{\omega_1}
\newcommand{\num}{\omega}
\newcommand{\den}{\bar{\omega}}
\newcommand{\numo}{\omega_0}
\newcommand{\dena}{\bar{\omega}_1}
\newcommand{\deno}{\bar{\omega}_0}

\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}
\theoremstyle{condition}
\newtheorem*{condition}{Condition}
\newtheorem{definition}{Definition}


\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}

\newcommand{\fairs}{FaiRS\xspace}

==> Tables/Personal-Loans/applicantSummaryStatistics-table.tex <==
\begin{tabular}{ l | c c c c c c c }
    & \multicolumn{5}{c}{\textbf{Quantiles}} \\
    & 1\% & 5\% & 25\% & 50\% & 75\% & 95\% & 99\% \\
    \hline 
    & \multicolumn{5}{c}{\textbf{All Applications}} \\
    Total Net Income (\$AU)  & 15,599 & 20,672 & 32,039 & 41,370 & 53,831 & 86,984 & 135,191 \\
    Total Liabilities (\$AU)  & -341 & 0 & 0 & 2 & 6,700 & 225,195 & 546,982 \\
    Credit Bureau Score & 0	& 0 & 443 & 587 & 689 & 827 & 936 \\
    & \multicolumn{5}{c}{\textbf{Funded Applications}} \\
    Total Net Income (\$AU)  & 17,316 & 22,439 & 33,095 & 41,471 & 53,111 & 83,891 & 118,922 \\
    Total Liabilities (\$AU)  & -943 & 0 & 0 & 0 & 7,000 & 262,628 & 539,278 \\
    Credit Bureau Score & 367 & 464 & 586 & 661 & 741 & 863	& 958 \\
    & \multicolumn{5}{c}{\textbf{Disadvantaged Geographic Areas}} \\
    Total Net Income (\$AU) & 15,323 & 19,913 & 30,227 & 39,107 & 50,735 & 80,303 & 127,391 \\
    Total Liabilities (\$AU) & -203 & 0 & 0 & 0 & 5,650 & 162,000 & 420,000 \\
    Credit Bureau Score & 0 & 0 & 406 & 566 & 677 & 828 & 937 \\
    & \multicolumn{5}{c}{\textbf{Non-disadvantaged Geographic Areas}} \\
    Total Net Income (\$AU)  & 15,600 & 20,796 & 32,435 & 41,858 & 54,625 & 88,595 & 137,005 \\
    Total Liabilities (\$AU) & -389 & 0 & 0 & 3 & 7000 & 246,000 & 572,007 \\
    Credit Bureau Score & 0 & 0 & 454 & 593 & 692 & 826 & 935 
\end{tabular}


==> Tables/Personal-Loans/loanPurpose-top10-table.tex <==
\begin{tabular}{l | c}
    \textbf{Loan Purpose} & \\
    \hline
    Used car & 31.6\% \\
    Refinance debt at other financial institution & 11.3\% \\
    Personal goods & 9.8\% \\
    Travel & 8.8\% \\
    New car & 6.2\% \\
    Other & 5.5\% \\
    Home Improvement & 5.1\% \\
    Other motor vehicle & 2.8\% \\
    Motor vehicle repairs & 2.8\% \\
    Land purchase & 2.5\%
\end{tabular}





==> Tables/Personal-Loans/loanTermSummaryStatistics-table.tex <==
\begin{tabular}{l | c c c c c c c}
    & \multicolumn{5}{c}{\textbf{Quantiles}} \\
    & 1\% & 5\% & 25\% & 50\% & 75\% & 95\% & 99\% \\
    \hline
    Loan size (\$AU) & 4,000 & 4,000 & 5,000 & 10,000 & 17,800 & 35,000 & 50,000 \\
    Interest rate & 8.49 & 11.9 & 13.9 & 13.9 & 15.9 & 17.9	& 18.4 \\
    Loan size to net income ratio & 0.056 & 0.081 & 0.139 & 0.238 & 0.412 & 0.793 & 1.150 \\
    Savings balance to loan size ratio & 0.000 & 0.000 & 0.026	& 0.087 & 0.267 & 1.339 & 4.374 
\end{tabular}
